Online Dynamic Pricing for Electric Vehicle Charging Stations with Reservations

This paper introduces a novel model for online dynamic pricing of electric vehicle charging services that integrates reservation, parking, and charging into a comprehensive bundle priced as a whole. Our approach focuses on the individual high-demand, fast-charging location, employing a Poisson process as a model of charging reservation arrivals, and develops an online dynamic pricing strategy optimized through a Markov Decision Process (MDP). A key contribution is the novel analysis of discretization error introduced when incorporating the continuous-time Poisson process into the discrete MDP framework. The MDP model's feasibility is demonstrated with a heuristic dynamic pricing method based on Monte-Carlo tree search, offering a viable path for real-world applications.

==> acronyms.tex <==
% Set glossaries hyperlinks to the text color, see https://tex.stackexchange.com/a/392724/45744
\makeatletter
\newcommand*{\glsplainhyperlink}[2]{%
    \begingroup%
      \hypersetup{hidelinks}%
      \hyperlink{#1}{#2}%
    \endgroup%
}
\let\@glslink\glsplainhyperlink
\makeatother

\makeglossaries[abbreviations]
\setabbreviationstyle[acronym]{long-short}

% Acronyms

\newabbreviation{mdp}{MDP}{Markov Decision Process}
% Stuff below messes up spaces after, see https://tex.stackexchange.com/questions/31091/space-after-latex-commands
% \newcommand{\MDP}{\gls{mdp}}
\makeatletter
    \@ifdefinable{\MDP}{\def\MDP/{\gls{mdp}}} % Usage: \MDP/ - the / is needed to get the spacing behavior after correct
\makeatother

\newabbreviation{ev}{EV}{Electric Vehicle}
\makeatletter
    \@ifdefinable{\EV}{\def\EV/{\gls{ev}}} 
\makeatother


\newabbreviation{mcts}{MCTS}{Monte-Carlo tree search}
\makeatletter
\@ifdefinable{\MCTS}{\def\MCTS/{\gls{mcts}}}
\makeatother

\newabbreviation{vi}{VI}{Value Iteration}
\newabbreviation{cs}{CS}{Charging Station}
% \newabbreviation{vi}{VI}{Value Iteration}

\newabbreviation{nrm}{NRM}{Network Revenue Management}
\newcommand{\NRM}{\gls{nrm}}
\newabbreviation{rpdsp}{RPDSP}{resource-constrained product dynamic sequential pricing problem}
\newcommand{\RPDSP}{\gls{rpdsp}}

% Electrific Terms
\newabbreviation{csp}{CSO}{Charging Station Operator}
\newabbreviation{cso}{CSO}{Charging Station Operator}
\newabbreviation{dso}{DSO}{Distribution System Operator}
\newabbreviation{es}{ES}{Energy Supplier}
\newabbreviation{emsp}{EMSP}{Electric Mobility Service Provider}
\newabbreviation{iea}{IEA}{International Energy Agency}


% Math acronyms
\newabbreviation{pmf}{PMF}{Probability Mass Function}
\makeatletter
    \@ifdefinable{\pmf}{\def\pmf/{\gls{pmf}}} % probability mass function - discrete
\makeatother

\newabbreviation{pdf}{PDF}{Probability Density Function} % Probability density function - continous
\makeatletter
    \@ifdefinable{\pdf}{\def\pdf/{\gls{pdf}}}
\makeatother

% PRICING PROBLEM
\newcommand{\BDG}{\beta} % budget distribution
\newcommand{\bdg}{b}   % sampled budget
\newcommand{\price}{h}  % price
% \newcommand{\RCP}{A}    %recipe matrix
% products
\newcommand{\prd}{\vec{p}}  % product (vector of resources)
% \newcommand{\prdi}{p}       % index of the product
\newcommand{\PRD}{P}        % Set of allowed products
% resources
% \newcommand{\res}{r}
\newcommand{\RES}{R}

% % customers
% \newcommand{\cst}{b}
\newcommand{\CST}{d}

% demand and requests
% \newcommand{\dem}{d}
\newcommand{\DEM}{D}

% MDP
% states
%\newcommand{\state}{s}
\newcommand{\St}{S}
\newcommand{\TR}{\mathcal{T}}    % transitions
\newcommand{\Rw}{R}   % rewards
\newcommand{\A}{A}    % actions

\newcommand{\cpc}{\vec{c}}  % supply
\newcommand{\nextr}{\sigma} % supply

% Experiments
\newcommand{\rev}{\rho}     % revenue
\newcommand{\util}{\mu}     % resource usage
\newcommand{\ts}{\text{ts}} % simulation time series of requests

% From minimum
\global\long\def\rreq#1{\mathit{req}(#1)}
\global\long\def\rstart#1{\mathit{start}(#1)}
\global\long\def\rend#1{\mathit{end}(#1)}
\global\long\def\rpar#1{par(#1)}
\global\long\def\revenue{\rho}
\global\long\def\elasticity{\mathcal{E}}
\global\long\def\mdp{\Pi}
\global\long\def\idn{\mathds{1}}

% From AAMAS
% \global\long\def\rreq#1{\mathit{req}(#1)}
% \global\long\def\rstart#1{\mathit{start}(#1)}
% \global\long\def\rend#1{\mathit{end}(#1)}
\global\long\def\rchar#1{char(#1)}
% \global\long\def\revenue{\rho}
% \global\long\def\elasticity{\mathcal{E}}
% \global\long\def\mdp{\Pi}
% \global\long\def\idn{\mathds{1}}


